Instability of the kinematic state in the atmosphere of the hypergiant Rho Cas outside outburst

Observations of the yellow hypergiant Rho Cas obtained in 2007-2011 in a wide wavelength region with spectral resolution about 60000 have enabled studies of features of its optical spectrum in detail and brought to light previously unknown characteristics of the extended atmosphere of the star. The radial velocity measured from symmetric absorptions of metals varies with an amplitude of about +/-7 km/s around the systemic velocity Vsys=-47 km/s, due to low-amplitude pulsations of the atmospheric layers near the photosphere. At some times, a velocity gradient was found in deep atmospheric layers of the star. A slight velocity stratification in the stellar atmosphere was detected for the first time, manifested as a difference of 3-4 km/s in the velocities measured from absorption lines of neutral metals and of ions. The long-wavelength components of split absorptions of BaII, SrII, TiII, and other strong lines with low excitation potentials for their lower levels are distorted by nearby emission lines. It is suggested that the short-wavelength components, whose locations correspond to the narrow velocity range Vr(blue) from approximately -60 to -70 km/s, are formed in a circumstellar envelope; one component of the D~NaI doublet and the emission components of the FeII 6369.46 and 6432.68 ions are also formed there.

==> longtab.tex <==

\begin{longtable}{l llc@{\quad} @{\quad}l @{\quad}l @{\quad}l@{\quad}}
\caption{Отождествление линий, их остаточные интенсивности
              и лучевые скорости ${\rm V_r }$\,, км/сек в спектре
	      Cyg\,OB2 - ${\rm \No}$\,12. В скобках указан номер мультиплета
	      }      
\\ \hline
\endfirsthead
\hline
\multicolumn{6}{l}{Табл.\,1, продолжение} \\ \hline
\endhead
\hline
\multicolumn{6}{r}{продолжение на след. странице} \\ \hline
\endfoot
\hline
\endlastfoot
\hline
 Е & & ${\rm \lambda_{lab}}$ &  W$_{\lambda}$, \AA & r  & ${\rm V_r }$  \\
\hline

\hline
\end{longtable}	       			     
\label{lines}

